Toward Edge-Efficient Dense Predictions with Synergistic Multi-Task Neural Architecture Search

In this work, we propose a novel and scalable solution to address the challenges of developing efficient dense predictions on edge platforms. Our first key insight is that MultiTask Learning (MTL) and hardware-aware Neural Architecture Search (NAS) can work in synergy to greatly benefit on-device Dense Predictions (DP). Empirical results reveal that the joint learning of the two paradigms is surprisingly effective at improving DP accuracy, achieving superior performance over both the transfer learning of single-task NAS and prior state-of-the-art approaches in MTL, all with just 1/10th of the computation. To the best of our knowledge, our framework, named EDNAS, is the first to successfully leverage the synergistic relationship of NAS and MTL for DP. Our second key insight is that the standard depth training for multi-task DP can cause significant instability and noise to MTL evaluation. Instead, we propose JAReD, an improved, easy-to-adopt Joint Absolute-Relative Depth loss, that reduces up to 88% of the undesired noise while simultaneously boosting accuracy. We conduct extensive evaluations on standard datasets, benchmark against strong baselines and state-of-the-art approaches, as well as provide an analysis of the discovered optimal architectures.

==> fig/fig_tab.tex <==
\begin{figure}[t]
% \hspace{1em}
\parbox[t]{4cm}{\null
    % \includegraphics[width=\linewidth]{./img/dp_mtl_nas.png}
    % \caption{Relationships of DP, MTL, and NAS}
    % \label{fig:dp_mtl_nas}
    \begin{subfigure}[b]{0.42\linewidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{./img/ibn.png}
        % \vspace{0.1em}
        \caption*{{
            IBN \\
            \cite{mobilenetv2}}}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}[b]{0.42\linewidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{./img/ibn_fused.png}
        % \vspace{0.1em}
        \caption*{{Fused-IBN\\
        \cite{mobiledet,nahas,efficientnetv2}}}
    \end{subfigure}
    % \vspace{-0.8em}
    \caption{\textbf{IBN vs FusedIBN}
    % -- Visualization of IBN and FusedIBN blocks used in the search space for EMNAS, as well as in the found architectures such as those in Table \ref{tab:arch_found} and \ref{tab:arch_found_depth}.
        % -- description
    }
    \label{fig:ibn_v_fused}
}
\quad
\parbox[t]{7.8cm}{\null
    \centering
    \vskip-\abovecaptionskip
    \captionof{table}[t]{\textbf{Effect of MRE-loss.}
    We train a model for segmentation and depth prediction on CityScapes with and without MRE-loss, each for 3 different runs, then calculate the mean and standard deviation}%
    \label{tab:depth_mre}
    \vskip\abovecaptionskip
    % \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
    \begin{tabular}{@{}l|cccccc@{}}
        \toprule
        % Loss weights
        %     & Seg
        %     & \multicolumn{2}{c}{MAE} 
        %     & \multicolumn{2}{c}{MRE} 
        %     \\
        Loss function
            & mIoU
            & $\sigma\%$
            & MAE 
            & $\sigma\%$
            & MRE 
            & $\sigma\%$ \\
        \midrule
        Seg+MAE 
            & 38.6
            & 2.5
            & 0.01763 
            & 4.4
            & 0.3541
            & 4.1
            \\
        Seg+MAE+MRE
            & 38.9
            & 1.6
            & 0.01680
            & 1.9
            & 0.3237 
            & 0.5
            \\
        (\% change)
            & $\uparrow$0.8
            & $\downarrow$34
            & $\downarrow$4.7
            & $\downarrow$57
            & $\downarrow$8.6
            & $\downarrow$88
            \\
        \bottomrule
    \end{tabular}
    % } %\resizebox
}
\end{figure}


==> fig/nas_overview.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
% \includegraphics[width=\linewidth]{example-image-golden}
\includegraphics[width=\linewidth]{./img/teaser.png}
% \vspace{-0.8em}
\end{center}
\caption{
% 
\textbf{An overview of our joint NAS and MTL system} -- The framework uses multi-objective NAS to simultaneously discover optimal neural components suitable for multi-task dense predictions, while ensuring efficient edge inference. Additionally, we propose EfficientDeP as a strong baseline model, MRE-loss for improving depth estimation, and a balance-aware metric for better characterizing the performance of multi-task models. 
}
%Chris:  you may want to consider changing the presentation of Figure 1 (i.e. add more of a caption or move it to where you describe your method). In its current position on the first page with a small caption caption, it could be confusing to the reader.
\label{fig:nas_overview}
% \vspace{-0.8em}
\end{figure}

==> sec/X_TODO.tex <==
\todo{
\section{Review plan:}
\begin{itemize}
    \item abstract and story (double check ppl reviews)
    \item teaser
    \item text
    \item figs and tabs
\end{itemize}

\section{TODO:}
\begin{itemize}
    \item Add stats to Abstract
    \item Requirements!!!
        \begin{itemize}
        \item 8 pages, 20MB % Papers are limited to eight pages, including figures and tables, in the WACV style. Additional pages containing only cited references are allowed. 
        % \item the main paper is restricted to 20MB.
        \item Domain Conflicts %Conflict Responsibilities: It is the primary author's responsibility to ensure that all authors on their paper have registered their institutional conflicts into the submission system – CMT3 (see details under Domain Conflicts below). If a paper is found to have an undeclared or incorrect institutional conflict, the paper may be summarily rejected. To avoid undeclared conflicts, the author list is considered to be final after the submission deadline and no changes are allowed for accepted papers.
        \item Primary topic on CMT dictates App/Algo (also select it in the paper template) %Enter subject (topic) areas for your paper. You must include at least one primary area and up to 2 secondary areas. Your primary selection will determine whether your paper is submitted to the Applications or Algorithms tracks.
        \end{itemize}
    \item Cross check Eq references
    \item EDNAS vs EDMAS
    %
    \vspace{2em}
    %
    \item CVPR23-version
        \begin{itemize}
        \item Check new Lit Rev in 2022
        \item More qualitative images from cityscapes
        \end{itemize}
    \item Camera-ready
        \begin{itemize}
        \item Clean up references
        \item make all images pdf
        \end{itemize}
    \item Additional experiments
        \begin{itemize}
        \item Investigate low SN acc baseline NYU-v2
        \end{itemize}
    % \item Teaser: visualization of method system + small table like MTAN, EfficientDet. Helpful in intro and informative for reviewers too
    % \item Visualize found arch, either with Chunfeng’s script or manually
    % \item Illustration for how EMNAS differs from other methods
    % \item How changing metrics and objective function affect NAS results
    %
    %
    % \item For everyone:
    % \begin{itemize}
    %     \item Claims: Are the main claims reasonable?
    %     \item Paper title and names: Please vote for the one you like below or suggest new ones
    %     \begin{itemize}
    %         \item {[[3]]  EMNAS: Efficient Multi-task Neural Architecture Search}
    %         \item {[[1]]  EMTAS: Efficient Multi-Task Architecture Search}
    %         \item {[[1]]  EfficientDeP ([De]nse [P]redictions)}
    %         \item {[[0]]  EfficientMultiTask}
    %         \item {[[0]]  EfficientMT}
    %         \item {[[1]]  EfficientTasks}
    %         \item {[[1]]  EfficientDense}
    %         \item {[[1]]  EfficientMultiDenses}
    %         \item {[[0]]  MASDeP (Multi-task Architecture Search for Dense Predictions)}
    %         \item {[[1]]  HAM: [H]ardware-aware [A]rchitecture Search for [M]ulti-task Dense Predictions}
    %     \end{itemize}
    % \end{itemize}
    % % \item For Thanh:
    % \begin{itemize}
    %
\end{itemize}
}

==> sec/X_introduction0.tex <==
\section{Introduction: 1.5p}
\label{sec:intro}
%%% THERE ARE GROWING DEMANDS FOR ON-EDGE DENSE PREDICTIONS
Recent years have witnessed a strong integration of computer vision in many downstream edge applications such as autonomous driving \cite{waymo_open,self_supervised_pillar_motion,cross_modality_3d,fusion_transformer,simple_det}, mobile vision \cite{fbnet,chamnet,mobilenets,mobilenetv3}, robotics \cite{robotics,yolactedge,rt_seg_fast_attention}, and precision agriculture \cite{Chiu_2020_CVPR,Kamilaris2018DeepLI,robot_cabbage}, fueled by rapid innovations of deep neural networks.
In many of these applications, pixel-level dense prediction tasks such as semantic segmentation or depth estimation can play a critical role.
For example, self-driving agents are using semantic and depth information to detect lanes, avoid obstacles, as well as locating their own positions.
In computational agriculture, output of these tasks can be used for crop analysis and yield prediction, or to help in-field robots navigate.
Thus, there has been continuously growing interest in developing edge-efficient architectures for dense predictions over the years as more and more neural models are being deployed into the real world.

%%% HOWEVER ON-EDGE DENSE PREDICTIONS ARE HARD
However, designing fast and efficient dense prediction models for edge devices are challenging.
%%% SPEED
First of all, pixel-level predictions such as semantic segmentation and depth estimation are fundamentally slower than some other popular vision tasks, including image classification or object detection.
This is because after encoding the input images into low-spatial resolution features, these networks need to upsample them back to produce high-resolution output masks.
In fact, dense estimation can be several times or even an order of magnitude slower than their counterparts, depending on the specific model, hardware, and target resolution.
Thus, not only that designing real-time dense predictions is non-trivial, these models can easily become a latency bottleneck in systems that utilize their outputs.
Such problems are intensified for edge applications on  platforms like the Coral TPU \cite{coral_edgetpu} due to the limited computational resources despite the need for low latency, e.g. to inform the users or process subsequent tasks.
% \todo{Fast dense prediction is critical in real systems because it's bottleneck other. no matter how faster the detectors are, it needs to wait for the segmentation results}

%%% SCALABILITY
Second, developing models for these edge environments is costly and hard to scale in practice. 
On one hand, the architectural design process requires significant amount of time, human labor, and expertise, with the development process ranging from a few months to a couple of years.
On the other hand, edge applications may require deployment on various platforms, including cellphones, robots, drones, and more. Unfortunately, optimal designs discovered for one hardware may not generalize to another.
All of these together pose challenges to the development of fast and efficient models for on-edge dense predictions.


%%% OUR SOLUTION
% Our solution is powered by (1) a novel joint learning of multi-task dense predictions (MT-DP) and hardware-aware neural architecture search (HwA-NAS), and (2) several technical insights and contributions that further enhance the efficacy of our system.
To address these problems, we propose a novel and scalable solution that performs joint optimization of multi-task learning of dense predictions (MTL-DP) and hardware-aware neural architecture search (HA-NAS).
%
Our key insight is that these two components when learned jointly are beneficial not only to the development of dense predictions on edge but also to each other. 
%
Our key idea is that we can leverage multi-task inference to significantly and linearly reduce computational costs across several dense prediction tasks, while utilize hardware-aware NAS to simultaneously mitigate negative transfer due to MTL, improve edge latency, and scale up the development process by both aiding the architecture design process and adapting to various edge platforms. \todo{Fig X illustrates this idea.}
%
Surprisingly, such combination is heavily understudied by the current literature. One on hand, state-of-the-art methods for multi-task dense predictions 

With regard to the latency requirement, multi-task models \cite{survey_mt_dense} that output several predictions at once is attractive as they avoid multiple inference runs and improve the overall speed by design.
However, improper sharing in multi-task architecture can lead to performance degradation.
Moreover, most existing methods for MT-DP study large models tar getting powerful graphic accelerators such as V100 GPU and are not readily suitable for edge applications. 
Our solution tackles these issues simultaneously using hardware-aware, multi-objective NAS to uncover efficient architectures with both improved accuracy and edge latency. 
In contrast to the current arts \cite{mtan,pcgrad,adashare,single_tasking_attentive,learning2branch,bmtas,branched_mt} that learn \textit{how to share layers} given a fixed network, 
our framework focuses on the question of \textit{what layers to use} to construct such MT-DP architecture in the first place 
given a fixed sharing strategy (e.g. hard parameter sharing)
and utilizes NAS to efficiently search for the optimal ones.
% We observe that EfficientDeP models trained with MRE-loss can perform $35\%$ better on CityScapes than DeepLab-ResNet-based models  \cite{deeplab_v2_2017,resnet}, have 1/4th the FLOP counts, and can act as strong baselines for evaluating multi-task dense prediction models.
\todo{Consider a table that ticks all the feature compare to DP, MT, NAS.}

Secondly, 
% through our analysis, we discover several novel technical insights of potential pitfalls and propose appropriate technical solutions to further enhance our framework. The proposed techniques are surprisingly effective while remaining straightforward and easy-to-adopt. 
% (A) 
Despite absolute error and relative error being the two most commonly used evaluation metrics for depth estimation, state-of-the-art MT-DP methods typically train with only MAE loss. This results in undesired noise caused by relative errors with large variance and in turn affect the evaluation of multi-task models. We propose the use of MRE loss as a simple but surprisingly effective augmentation to simultaneously improve prediction accuracy by 40\% and reduce negative effect of relative error noise by 10$\times$.
%% should I claim the weak-strong EfficientDeP insight here?
% (B) 
% We observe a growing trend in utilizing the average improvement across all tasks as a summary metric for multi-task performance. Although this is certainly useful, especially for large number of tasks, a mean-only evaluation strategy is insufficient and could mask away potentially severe model bias, even accuracy drop, caused by imbalanced multi-task training. We argue that a good multi-task models should improve performance uniformly across all tasks. Thus, we propose a simple augmentation of the evaluation process by considering the variance or standard deviation of per-task improvement, yielding a \textit{balance-aware} metric system.

To summarize our contributions, 
\begin{itemize}
    % \item We propose Efficient Multi-Task Neural Architecture Search (EMNAS),
    % % a framework that deploys hardware-aware NAS to discover efficient multi-task models for dense predictions on edge devices.
    % % We show that direct searching of multi-task architectures yields better results than the transferring of searched single-task architectures.
    % one of the first attempts, to the best of our knowledge, at applying standard NAS to search for the layer types of multi-task dense prediction networks.
    % \item We introduce EfficientDeP, an extension of the EfficientNet \cite{efficientnetv1} family to multi-task dense predictions
    % and propose the use of MRE loss for depth estimation.
    % % to improve relative error and reduce noise in multi-task evaluation. 
    % % We observe that EfficientDeP is a strong baseline for multi-task dense predictions, and apply EMNAS to obtain even more improvement.
    % \item We propose to use \textit{balance-aware} metrics such as the standard deviation of per-task improvements to quantify and summarize models' ability to balance task learning.
    % % Yanqi Zhou: Better to mention that our meta-objective (reward) enables directly optimizing the balance-aware metric. Mention the concrete gains here.
    % % to capture the variance in per-task improvements and characterize how multi-task model balance the learning across all tasks.
    \item (1)+(2) Scalable and edge-targeted model design => Joint learning Multitask + NAS. Edge-friendlier baseline architecture => EfficientDeP
    \item (3) Improved depth learning => MRE loss. maybe not (4) Improved evaluation => Balance-aware metric => part of evaluation study
    \item We conduct experiments on CityScapes \cite{cityscapes} and show that EfficientDeP is 35\% more accurate than baseline models used by previous works and EMNAS can further improve \textit{both} accuracy (+3\%) and speed (+6\%).
    % using popular datasets and show significant improvement in terms of both accuracy and speed.
\end{itemize}

% We propose the tangent image spherical representation: a set of oriented, low-distortion images rendered
% tangent to faces of the icosahedron.
%  We show that standard CNNs trained on tangent images perform competitively with specialized spherical
% convolutional kernels while also scaling effectively to
% high resolution spherical images.
%  We demonstrate that tangent images facilitate network
% transfer between perspective and spherical images with
% no fine tuning and minimal performance drop-off.
%  We illustrate the utility of tangent images for traditional computer vision tasks by using them to improve
% sparse keypoint matching on spherical images.

==> sec/X_metadata.tex <==
% \renewcommand\thelinenumber{\color[rgb]{0.2,0.5,0.8}\normalfont\sffamily\scriptsize\arabic{linenumber}\color[rgb]{0,0,0}}
% \renewcommand\makeLineNumber {\hss\thelinenumber\ \hspace{6mm} \rlap{\hskip\textwidth\ \hspace{6.5mm}\thelinenumber}}
% \linenumbers
\pagestyle{headings}
\mainmatter
\def\ECCVSubNumber{100}  % Insert your submission number here

\title{
EMNAS: Efficient Multi-Task Neural Architecture Search for Dense Predictions
} % Replace with your title

% INITIAL SUBMISSION 
%\begin{comment}
\titlerunning{ECCV-22 submission ID \ECCVSubNumber} 
\authorrunning{ECCV-22 submission ID \ECCVSubNumber} 
\author{Anonymous ECCV submission}
\institute{Paper ID \ECCVSubNumber}
%\end{comment}
%******************

% CAMERA READY SUBMISSION
\begin{comment}
\titlerunning{Abbreviated paper title}
% If the paper title is too long for the running head, you can set
% an abbreviated paper title here
%
\author{First Author\inst{1}\orcidID{0000-1111-2222-3333} \and
Second Author\inst{2,3}\orcidID{1111-2222-3333-4444} \and
Third Author\inst{3}\orcidID{2222--3333-4444-5555}}
%
\authorrunning{F. Author et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%
\institute{Princeton University, Princeton NJ 08544, USA \and
Springer Heidelberg, Tiergartenstr. 17, 69121 Heidelberg, Germany
\email{lncs@springer.com}\\
\url{http://www.springer.com/gp/computer-science/lncs} \and
ABC Institute, Rupert-Karls-University Heidelberg, Heidelberg, Germany\\
\email{\{abc,lncs\}@uni-heidelberg.de}}
\end{comment}
%******************

==> sec/X_notes.tex <==
Regularize Evolution:
We speculate that asynchronous evolution may be reducing the FLOPs because it is indirectly optimizing for speed even when training for a fixed number of epochs: fast models may do well because they “reproduce” quickly even if they initially lack the higher accuracy of their slower peers.
ing the algorithm to focus on it, reducing exploration. Under aging evolution (AE), on the other hand, all models have a short lifespan, so the population is wholly renewed frequently, leading to more diversity and more exploration. 
In addition, another effect may be in play, which we describe next. In AE, because models die quickly, the only way an architecture can remain in the population for a long time is by being passed down from parent to child through the generations. Each time an architecture is inherited it must be re-trained. If it produces an inaccurate model when retrained, that model is not selected by evolution and the architecture disappears from the population. The only way for an architecture to remain in the population for a long time is to re-train well repeatedly. In other words, AE can only improve a population through the inheritance of architectures that re-train well. (In contrast, NAE can improve a population by accumulating architectures/models that were lucky when they trained the first time). That is, AE is forced to pay attention to architectures rather than models. In other words, the addition of aging involves introducing additional information to the evolutionary process: architectures should retrain well. This additional information prevents overfitting to the training noise, which makes it a form of regularization in the broader mathematical sense

==> tab/2_gen_stronger_cityscapes0.tex <==
\begin{table*}[!t]
\centering

\caption{
\textbf{Stronger baselines for CityScapes} -- abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz abc xyz ...
} % \caption
\label{tab:2_gen_stronger_cityscapes}

\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}l|cc||cc|cc||cc|cc@{}}
\begin{tabular}{@{}lccc cccc cc|cc@{}}

\toprule

\multicolumn{1}{c}{}  
    & \multicolumn{3}{c}{Model} 
    & \multicolumn{2}{c}{Seg} 
    & \multicolumn{2}{c}{Depth} 
    & \multicolumn{4}{c}{Multi-Task Perf.} \\

Method 
    % & Arch 
    & GFLOPs 
    & Lat
    & Speedup%$\uparrow$ 
    & mIoU 
    & PAcc 
    & AbsE 
    & RelE 
    & $\Delta$Seg
    & $\Delta$Depth
    & Mean$\Delta$ 
    & STD$\Delta$ \\

\midrule

ST Res. baseline \cite{adashare}  
    % & Res. 
    & 66.70$^\dag$ 
    & ---
    & ---
    & 40.20  
    & 74.70  
    & .0170 
    & .330 
    & ---
    & ---
    & ---
    & ---\\
% MT Res. baseline \cite{adashare} 
%     % & Res. 
%     & 44.31 
%     & ---
%     & ---
%     & 37.70 
%     & 73.80 
%     & .0180 
%     & .340 
%     & -3.7 
%     & -4.5 
%     & -4.1 
%     & \underline{0.5} \\

% Cross-Stitch \cite{cross_stitch} 
%     % & Res. 
%     & 37.06   
%     & ---
%     & ---
%     & 40.30 
%     & 74.30 
%     & .0150 
%     & .300 
%     & -0.1 
%     & \textbf{+10.4} 
%     & \textbf{+5.1} 
%     & 7.5 \\

% Sluice \cite{sluice} 
%     % & Res. 
%     & 37.06  
%     & ---
%     & ---
%     & 39.80 
%     & 74.20 
%     & .0160 
%     & .310 
%     & -0.8 
%     & +6.0 
%     & +2.6 
%     & 4.8 \\

% NDDR-CNN \cite{nddr} 
%     % & Res. 
%     & 38.32  
%     & ---
%     & ---
%     & 41.50 
%     & 74.20 
%     & .0170 
%     & .310 
%     & +1.3 
%     & +3.0 
%     & +2.2 
%     & 1.2 \\

% MTAN \cite{mtan} 
%     % & Res. 
%     & 44.31  
%     & ---
%     & ---
%     & 40.80 
%     & 74.30 
%     & .0150 
%     & .320 
%     & +0.5 
%     & \underline{+7.4} 
%     & \underline{+3.9} 
%     & 4.9 \\
    
% DEN \cite{nas_mt_cls_elastic} 
%     % & Res. 
%     & 78.36$^\dag$  
%     & ---
%     & ---
%     & 38.00 
%     & 74.20 
%     & .0170 
%     & .370 
%     & -3.1 
%     & -6.1 
%     & -4.6 
%     & 2.1 \\

% AdaShare \cite{adashare} 
%     % & Res. 
%     & 66.70$^\dag$   
%     & ---
%     & ---
%     & 41.50 
%     & 74.90 
%     & .0160 
%     & .330 
%     & \underline{+1.8} 
%     & +2.9 
%     & +2.3 
%     & 0.8 \\

% \midrule

ST Res. baseline 
    % & Res. 
    & 78.85$^\dag$ 
    & 86.57
    & ---%$\times$1.0
    & 41.04 
    & 89.05 
    & .0168    
    & .359
    & ---   
    & ---
    & ---
    & --- \\
    
% MT Res. baseline 
%     % & Res. 
%     & 39.52
%     & 51.48
%     & $\times$1.7
%     & {37.66}
%     & {88.66}
%     & {.0175}
%     & {.371}
%     & -4.3	 
%     & -3.9	
%     & -4.1	
%     & 0.3 \\

% % ST EfficientDeP
% %     % & Eff. 
% %     & 4x 2.34$^\dag$ 
% %     &  25.67
% %     & ---
% %     & 40.04	
% %     & 88.68
% %     & .0157  
% %     & .340 
% %     & -1.4	
% %     & +5.7	
% %     & +2.1	
% %     & \todo{5.0}\\ % should I improve this?
    
% EfficientDeP
%     % & Eff. 
%     & 4.78
%     & 20.82
%     & $\times$4.2
%     & 38.64	 
%     & 88.49	
%     & .0171	
%     & .354 
%     & -3.2	
%     & -0.2	
%     & -1.7	
%     & 2.1\\

% EdgeDeP
%     % & Eff. 
%     & 16.50
%     & 20.29
%     & $\times$4.3
%     & 46.52	
%     & 90.61	
%     & .0143	
%     & .316
%     & +7.5		
%     & +13.1
%     & +10.3	
%     & 3.9\\ 

% EdgeDeP+MRE
%     &&&&&&&&&&&\\

% EdgeDeP+MRE+BAM
%     &&&&&&&&&&&\\

    
% +MRE
%     % & Eff. 
%     & {8.25}  
%     & 20.21
%     & ---
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}\\ 

% +BAM/BAE rewei
%     % & Eff. 
%     & {8.25}  
%     & 20.21
%     & ---
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}\\ 

% \midrule
% \midrule

ST EfficientDeP
    % & Eff. 
    & 9.37$^\dag$ 
    & 25.67
    & ---%$\times$1.0
    & 40.04	
    & 88.68
    & .0157  
    & .340 
    & ---
    & ---
    & ---
    & ---\\
% MT EfficientDeP
%     % & Eff. 
%     & 4.78
%     & 20.82
%     & $\times$1.2
%     & 38.64	 
%     & 88.49	
%     & .0171	
%     & .354 
%     & -1.9	
%     & -6.3	
%     & -4.1	
%     & 3.1\\
    
% \\

% EdgeDeP 
%     % & Eff. 
%     & 16.50
%     & 20.29
%     & $\times$1.3
%     & 46.52	
%     & 90.61	
%     & .0143	
%     & .316
%     & +9.2	
%     & +7.9	
%     & +8.5	
%     & 0.9\\ 
% % EdgeDeP+MRE
% %     % & Eff. 
% %     & 16.50
% %     & 20.29
% %     & $\times$1.3
% %     & 42.36	
% %     & 89.91	
% %     & .0145	
% %     & .232
% %     & +3.6	
% %     & +19.7		
% %     & +11.7		
% %     & 11.4\\ 
% EdgeDeP+MRE
%     % & Eff. 
%     & 16.50
%     & 20.29
%     & $\times$1.3
%     & 45.33	
%     & 90.41	
%     & .0141	
%     & .282
%     & +7.6
%     & +13.8	
%     & +10.7		
%     & 4.4\\ 
% EdgeDeP+MRE+BAM
%     & 16.50
%     & 20.29
%     & $\times$1.3
%     & 46.82		
%     & 90.58		
%     & .0141	
%     & .312
%     & +9.5		
%     & +9.4		
%     & +9.5		
%     & 0.1\\ 

% \\
    
% EfficientDeP+MRE
%     % & Eff. 
%     & 4.78
%     & 20.82
%     & $\times$1.2
%     & 37.71	
%     & 88.49
%     & .0161
%     & .324
%     & -3.0	
%     & +1.3	
%     & -0.9	
%     & 3.0\\

% EfficientDeP+MRE+BAM
%     % & Eff. 
%     & 4.78
%     & 20.82
%     & $\times$1.2
%     & 38.89
%     & 88.63
%     & .0168	
%     & .324
%     & -1.5	
%     & -0.9	
%     & -1.2	
%     & 0.4\\

% EdgeDeP+MRE+BAM
%     % & Eff. 
%     & 16.50
%     & 20.29
%     & $\times$1.3
%     & 46.82		
%     & 90.58		
%     & .0141	
%     & .312
%     & +9.5		
%     & +9.4		
%     & +9.5		
%     & 0.1\\ 

\midrule

ST EfficientDeP
    % & Eff. 
    & 9.37$^\dag$ 
    & 25.67
    & ---%$\times$1.0
    & 55.02	
    & 92.29	
    & .0116	 
    & .168
    & ---
    & ---
    & ---
    & ---\\
MT EfficientDeP
    % & Eff. 
    & 4.78
    & 20.82
    & $\times$1.2
    & 53.80	
    & 91.94	
    & .0124	
    & .159
    & -1.3	
    & -0.9	
    & -1.1	
    & 0.3\\
EdgeDeP+MRE+BAM
    % & Eff. 
    & 9.37$^\dag$ 
    & 25.67
    & $\times$1.3
    & 58.54	
    & 92.78	
    & .0117	
    & .156
    & +3.5	
    & +3.1	
    & +3.3	
    & 0.3\\

\bottomrule
\end{tabular}
} % \resizebox
\end{table*}

==> tab/ablations.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Ours v0 & Frumpy \\
Ours v1 & Frobbly \\
\textbf{Ours} & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
\textbf{Ablations} -- our decisions are well justified.
% 
} % \caption
\label{tab:ablations}
\end{table}

==> tab/latency.tex <==
\begin{table}
\centering

\caption{
\textbf{Computation costs and latency on Coral EdgeTPU \cite{coral_edgetpu}
} % -- Text description here
%NAS improvement from the summer: 30ms => 21ms
} % \caption
\label{tab:latency}

% \resizebox{0.7\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccccc@{}}
\toprule
Method 
    & \#P
    & FLOPs 
    & Lat 
    % & \%Lat
    & $\Delta T_{all}$ 
    \\
    
\midrule

ST Resnet-ASPP \cite{adashare}
    & 42.6
    & 87.12 %87.12 %66.70$^\dag$ 
    & ---
    % & ---
    & ---
    \\
% MT Resnet-ASPP \cite{adashare} 
%     & 21.3
%     & 43.56
%     & ---
%     \\
ST Resnet-BiFPN
    & 43.7
    & 19.71
    & 86.57
    % & +316
    & 0
    \\
    
MT Resnet-BiFPN  
    & 21.9
    & 9.88
    & 51.48
    % & +147
    & -4.1
    \\
    
% ST Efficientnet-BiFPN  
%     & 6.8
%     & 2.34
%     & 25.67 ms
%     \\

MT Efficientnet-BiFPN
    & 3.4
    & 1.20
    & 20.82
    % & 0
    & -4.1
    \\
    
EDNAS %EMNAS (p=0,q=-.07)          
    & 4.3
    & 4.12
    & \textbf{20.29}
    % & \textbf{-2.5}
    & \textbf{+8.5}
    \\
\bottomrule
\end{tabular}
% } % \resizebox
% \vspace{-2em}
\end{table}



% \begin{table}
% \centering
% \resizebox{0.7\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% Method & FLOPs & \#Params & Mean$\Delta$ & Latency \\
% \midrule
% ST EfficientDeP & 4.69G & 3.42M & 0.0 & 25.5 ms \\
% MT EfficientDeP & 2.39G & 3.43M & -1.1 & 20.8 ms\\
% EMNAS (p=0,q=-.07)          & 8.25G & 4.32M & \textbf{+3.3} & \underline{20.2} ms\\
% EMNAS (p=q=-.07)  & 4.97G & 3.55M & \underline{+3.0} & \textbf{19.5} ms\\
% \bottomrule
% \end{tabular}
% } % \resizebox
% \caption{
% \textbf{Latency on Coral EdgeTPU \cite{coral_edgetpu} 
% \todo{move to ablation}
% } % -- Text description here
% %NAS improvement from the summer: 30ms => 21ms
% } % \caption
% \label{tab:latency}
% % \vspace{-2em}
% \end{table}

==> tab/loss_weight_impact2.tex <==
\begin{table*}[t]
    \centering
    % \vspace{-1em}
    \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
    \begin{tabular}{@{}l|cccc|cc|c@{}}
    \toprule
    $\mathcal{L}_{CE}:\mathcal{L}_{1}:\mathcal{L}_{RE}$
        & mIoU 
        & PAcc 
        & AbsE 
        & RelE
        % & $\Delta$mIoU 
        % & $\Delta$PAcc 
        % & $\Delta$AbsE 
        % & $\Delta$RelE
        & $\Delta T_{S}$
        & $\Delta T_{D}$
        & $\Delta T$
        \\
    \midrule
    1.0:0.000:0.000
        & 40.04 
        & 88.68
        & ---  
        & --- 
        % & 16.8
        % & 2.2
        % & 5.4
        % & 4.8
        & --- 
        & ---
        & ---
        \\
    0.0:1.000:0.000
        & ---
        & ---
        & 0.0157  
        & 0.340 
        % & 16.8
        % & 2.2
        % & 5.4
        % & 4.8
        & --- 
        & ---
        & ---
        \\
    0.5:1.000:0.000
        & 38.64
        & 88.49 
        & 0.0171 
        & 0.354
        % & 16.8
        % & 2.2
        % & 5.4
        % & 4.8
        & -1.9 
        & -6.3 
        & -4.1
        \\
    0.5:0.999:0.001
        & 46.78
        & 90.62
        & 0.0149
        & 0.323
        % & 16.8
        % & 2.2
        % & 5.4
        % & 4.8
        & +9.5
        & +5.1
        & +7.3
        \\
    0.5:0.990:0.010
        & 46.83
        & 90.56	
        & 0.0144	
        & 0.304
        % & 17.0
        % & 2.1
        % & 8.6
        % & 10.4
        & +9.5
        & +9.5
        & +9.5
        \\
    0.5:0.950:0.050
        & 46.11	
        & 90.47	
        & 0.0143	
        & 0.281
        % & 15.1
        % & 2.0
        % & 9.1
        % & 17.4
        & +8.6
        & +13.3
        & +10.9
        \\
    0.5:0.900:0.010
        & 46.41	
        & 90.56	
        & 0.0146	
        & 0.300
        % & 15.9
        % & 2.1
        % & 7.5
        % & 11.6
        & +9.0
        & +9.5
        & +9.3
        \\
    \bottomrule
    \end{tabular}
    } % \resizebox
    \caption{
        \textbf{Impact of loss weighting}
    } % \caption
    \label{tab:loss_weight_impact}
\end{table*}


==> tab/loss_weight_impact3.tex <==
% \FloatBarrier
% \begin{wraptable}{o}{0.1cm}
\begin{table*}[t]
    \centering
    % \vspace{-1em}
    \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
    \begin{tabular}{@{}ccc|cccc|cc|c@{}}
    \toprule
    % \multicolumn{1}{c}{}  
    %     &\multicolumn{1}{c}{} 
    %     & \multicolumn{1}{c}{Seg} 
    %     & \multicolumn{2}{c}{Depth} 
    %     & \multicolumn{1}{c}{SN}%{Surf. Normal}
    %     \\
    $\mathcal{L}_{CE}$
        & $\mathcal{L}_{1}$
        & $\mathcal{L}_{RE}$
        & mIoU 
        & PAcc 
        & AbsE 
        & RelE
        % & $\Delta$mIoU 
        % & $\Delta$PAcc 
        % & $\Delta$AbsE 
        % & $\Delta$RelE
        & $\Delta T_{S}$
        & $\Delta T_{D}$
        & $\Delta T$
        \\
    \midrule
    1.000
        & 0.000
        & 0.000
        %%
        & 40.04 
        & 88.68
        & ---  
        & --- 
        % & 16.8
        % & 2.2
        % & 5.4
        % & 4.8
        & --- 
        & ---
        & ---
        \\
    0.000 & 1.000 & 0.000
        & ---
        & ---
        & 0.0157  
        & 0.340 
        % & 16.8
        % & 2.2
        % & 5.4
        % & 4.8
        & --- 
        & ---
        & ---
        \\
    0.500 & 1.000 & 0.000
        & 38.64
        & 88.49 
        & 0.0171 
        & 0.354
        % & 16.8
        % & 2.2
        % & 5.4
        % & 4.8
        & -1.9 
        & -6.3 
        & -4.1
        \\
    0.500 & 0.999 & 0.001
        & 46.78
        & 90.62
        & 0.0149
        & 0.323
        % & 16.8
        % & 2.2
        % & 5.4
        % & 4.8
        & +9.5
        & +5.1
        & +7.3
        \\
    0.500 & 0.990 & 0.010
        & 46.83
        & 90.56	
        & 0.0144	
        & 0.304
        % & 17.0
        % & 2.1
        % & 8.6
        % & 10.4
        & +9.5
        & +9.5
        & +9.5
        \\
    0.500 & 0.950 & 0.050
        & 46.11	
        & 90.47	
        & 0.0143	
        & 0.281
        % & 15.1
        % & 2.0
        % & 9.1
        % & 17.4
        & +8.6
        & +13.3
        & +10.9
        \\
    0.500 & 0.900 & 0.010
        & 46.41	
        & 90.56	
        & 0.0146	
        & 0.300
        % & 15.9
        % & 2.1
        % & 7.5
        % & 11.6
        & +9.0
        & +9.5
        & +9.3
        \\
    \bottomrule
    \end{tabular}
    } % \resizebox
    \caption{
        \textbf{Impact of loss weighting}
    } % \caption
    \label{tab:loss_weight_impact}
\end{table*}
% \end{wraptable}
% \FloatBarrier

==> tab/main_table.tex <==
\begin{table*}[!t]
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}l|cc||cc|cc||cc|cc@{}}
\toprule
        \multicolumn{1}{c}{}  &\multicolumn{2}{c}{Model} & \multicolumn{2}{c}{Seg} & \multicolumn{2}{c}{Depth} & \multicolumn{4}{c}{Relative Multi-Task Performance} \\
Method & Arch & GFLOPs & mIoU & PixAcc & AbsE & RelE & $\Delta$Seg(v.*) & $\Delta$Depth(v.*) & Mean$\Delta$ & STD$\Delta$ \\

\midrule
ST baseline* \cite{adashare}  & Res. &
    66.70$^\dag$     & 40.2  & 74.7  & 0.0170 & 0.330 & 0.0    & 0.0    & 0.0   & 0.0\\
MT baseline \cite{adashare} & Res. &
    44.31 &37.70 & 73.80 & 0.0180 & 0.340 & -3.7 & -4.5 & -4.1 & \underline{0.5} \\

Cross-Stitch \cite{cross_stitch} & Res. & 
    37.06   & 40.30 & 74.30 & 0.0150 & 0.300 & -0.1 & \textbf{+10.4} & \textbf{+5.1} & 7.5 \\

Sluice \cite{sluice} & Res. &
    37.06  & 39.80 & 74.20 & 0.0160 & 0.310 & -0.8 & +6.0 & +2.6 & 4.8 \\

NDDR-CNN \cite{nddr} & Res. &
    38.32  & 41.50 & 74.20 & 0.0170 & 0.310 & +1.3 & +3.0 & +2.2 & 1.2 \\

MTAN \cite{mtan} & Res. &
    44.31  & 40.80 & 74.30 & 0.0150 & 0.320 & +0.5 & \underline{+7.4} & \underline{+3.9} & 4.9 \\
    
DEN \cite{nas_mt_cls_elastic} & Res. &
    78.36$^\dag$  & 38.00 & 74.20 & 0.0170 & 0.370 & -3.1 & -6.1 & -4.6 & 2.1 \\

AdaShare \cite{adashare} & Res. &
    66.70$^\dag$   & 41.50 & 74.90 & 0.0160 & 0.330 & \underline{+1.8} & +2.9 & +2.3 & 0.8 \\

\midrule
ST EfficientDeP & Eff. &
    \underline{4.69}$^\dag$  & \underline{55.02} & \underline{92.29} & \textbf{0.0116}   & 0.168 & 0.0 (+30)    & 0.0 (+41) & 0.0 (+35)   & 0.0 \\
% ST EfficientDeP & Eff. &
%     \underline{4.69}$^\dag$  & \underline{55.02} & \underline{92.29} & \textbf{0.01155}   & 0.1681 & --- (+30)    & --- (+41) & --- (+35)   & --- \\
MT EfficientDeP & Eff. &
    \textbf{2.39}  & 53.80	& 91.94	& {0.0124} & \underline{0.159} & -1.3 (+28)  & -0.9 (+39) & -1.1 (+34) & \textbf{0.3}\\
EMNAS & Eff. &
    {8.25}  & \textbf{58.54} & \textbf{92.78} & \underline{0.0117}   & \textbf{0.156} & \textbf{+3.5} (\textbf{+35}) & {+3.1 (\textbf{+42})} & {+3.3 (\textbf{+38})} & \textbf{0.3}\\ 
\bottomrule
\end{tabular}
} % \resizebox
\caption{
\textbf{CityScapes results for 19-class semantic segmentation and depth estimation} -- Best numbers are in \textbf{bold}, second best are \underline{underlined}. Measurements of prior works are from Table 8 and Table 11 in \cite{adashare}. The parameter count for our single-task EfficientDeP is 3.42M. \textit{ST} stands for single-tasks. \textit{MT} stands for multi-task. We multiply the FLOPs by the number of tasks for methods that need multiple runs to get different per-task predictions.
% $^\dag$ means the measurement were summed over all tasks because the network performs one task at a time.
% \todo{(TODO: Update the description)} 
} % \caption
\label{tab:main_table}
% \vspace{-0.5em}
\end{table*}

==> tab/sota.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
% 
\textbf{State of the art} -- Glory to the bold numbers.
% 
} % \caption
\label{tab:sota}
\end{table}

==> tab/sota_cityscapes0.tex <==
\begin{table*}[!t]
\centering

\caption{
\textbf{CityScapes results for 19-class semantic segmentation and depth estimation} -- Best numbers are in \textbf{bold}, second best are \underline{underlined}. Measurements of prior works are from Table 8 and Table 11 in \cite{adashare}. The parameter count for our single-task EfficientDeP is 3.42M. \textit{ST} stands for single-tasks. \textit{MT} stands for multi-task. We multiply the FLOPs by the number of tasks for methods that need multiple runs to get different per-task predictions.
% $^\dag$ means the measurement were summed over all tasks because the network performs one task at a time.
} % \caption
\label{tab:main_table}

\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}l|cc||cc|cc||cc|cc@{}}
\begin{tabular}{@{}lccc cccc cc|cc@{}}

\toprule

\multicolumn{1}{c}{}  
    & \multicolumn{3}{c}{Model} 
    & \multicolumn{2}{c}{Seg} 
    & \multicolumn{2}{c}{Depth} 
    & \multicolumn{4}{c}{Multi-Task Perf.} \\

Method 
    % & Arch 
    & GFLOPs 
    & Lat
    & Speedup%$\uparrow$ 
    & mIoU 
    & PAcc 
    & AbsE 
    & RelE 
    & $\Delta$Seg
    & $\Delta$Depth
    & Mean$\Delta$ 
    & STD$\Delta$ \\

\midrule

ST Res. baseline \cite{adashare}  
    % & Res. 
    & 66.70$^\dag$ 
    & ---
    & ---
    & 40.20  
    & 74.70  
    & .0170 
    & .330 
    & ---
    & ---
    & ---
    & ---\\
MT Res. baseline \cite{adashare} 
    % & Res. 
    & 44.31 
    & ---
    & ---
    & 37.70 
    & 73.80 
    & .0180 
    & .340 
    & -3.7 
    & -4.5 
    & -4.1 
    & \underline{0.5} \\

Cross-Stitch \cite{cross_stitch} 
    % & Res. 
    & 37.06   
    & ---
    & ---
    & 40.30 
    & 74.30 
    & .0150 
    & .300 
    & -0.1 
    & \textbf{+10.4} 
    & \textbf{+5.1} 
    & 7.5 \\

Sluice \cite{sluice} 
    % & Res. 
    & 37.06  
    & ---
    & ---
    & 39.80 
    & 74.20 
    & .0160 
    & .310 
    & -0.8 
    & +6.0 
    & +2.6 
    & 4.8 \\

NDDR-CNN \cite{nddr} 
    % & Res. 
    & 38.32  
    & ---
    & ---
    & 41.50 
    & 74.20 
    & .0170 
    & .310 
    & +1.3 
    & +3.0 
    & +2.2 
    & 1.2 \\

MTAN \cite{mtan} 
    % & Res. 
    & 44.31  
    & ---
    & ---
    & 40.80 
    & 74.30 
    & .0150 
    & .320 
    & +0.5 
    & \underline{+7.4} 
    & \underline{+3.9} 
    & 4.9 \\
    
DEN \cite{nas_mt_cls_elastic} 
    % & Res. 
    & 78.36$^\dag$  
    & ---
    & ---
    & 38.00 
    & 74.20 
    & .0170 
    & .370 
    & -3.1 
    & -6.1 
    & -4.6 
    & 2.1 \\

AdaShare \cite{adashare} 
    % & Res. 
    & 66.70$^\dag$   
    & ---
    & ---
    & 41.50 
    & 74.90 
    & .0160 
    & .330 
    & \underline{+1.8} 
    & +2.9 
    & +2.3 
    & 0.8 \\

\midrule

ST Res. baseline 
    % & Res. 
    & 78.85$^\dag$ 
    & 86.57
    & ---%$\times$1.0
    & 41.04 
    & 89.05 
    & .0168    
    & .359
    & ---   
    & ---
    & ---
    & --- \\
    
MT Res. baseline 
    % & Res. 
    & 39.52
    & 51.48
    & $\times$1.7
    & {37.66}
    & {88.66}
    & {.0175}
    & {.371}
    & -4.3	 
    & -3.9	
    & -4.1	
    & 0.3 \\

% ST EfficientDeP
%     % & Eff. 
%     & 4x 2.34$^\dag$ 
%     &  25.67
%     & ---
%     & 40.04	
%     & 88.68
%     & .0157  
%     & .340 
%     & -1.4	
%     & +5.7	
%     & +2.1	
%     & \todo{5.0}\\ % should I improve this?
    
EfficientDeP
    % & Eff. 
    & 4.78
    & 20.82
    & $\times$4.2
    & 38.64	 
    & 88.49	
    & .0171	
    & .354 
    & -3.2	
    & -0.2	
    & -1.7	
    & 2.1\\

EdgeDeP
    % & Eff. 
    & 16.50
    & 20.29
    & $\times$4.3
    & 46.52	
    & 90.61	
    & .0143	
    & .316
    & +7.5		
    & +13.1
    & +10.3	
    & 3.9\\ 

EdgeDeP+MRE
    & 16.50
    & 20.29
    & $\times$4.3
    & 
    & 
    & 
    & 
    & +8.6	
    & +8.3	
    & +8.4	
    & 0.2\\

EdgeDeP+MRE
    & 16.50
    & 20.29
    & $\times$4.3
    & 47.28	
    & 90.52	
    & .0161	
    & .298
    & +8.4	
    & +10.4	
    & +9.4	
    & 1.4\\

EdgeDeP+MRE
    & 16.50
    & 20.29
    & $\times$4.3
    & 
    & 
    & 
    & 
    & +8.9	
    & +11.6	
    & +10.2	
    & 1.9\\

EdgeDeP+MRE
    & 16.50
    & 20.29
    & $\times$4.3
    & 
    & 
    & 
    & 
    & +7.0		
    & +18.2		
    & +12.6	
    & 7.9\\
    
% EdgeDeP+MRE+$p_{seg}$
%     &&&&&&&&&&&\\

% EdgeDeP+MRE+$p_{depth}$
%     &&&&&&&&&&&\\
    
% +MRE
%     % & Eff. 
%     & {8.25}  
%     & 20.21
%     & ---
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}\\ 

% +BAM/BAE rewei
%     % & Eff. 
%     & {8.25}  
%     & 20.21
%     & ---
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}
%     & \todo{todo}\\ 

\midrule
\midrule

ST EfficientDeP
    % & Eff. 
    & 9.37$^\dag$ 
    & 25.67
    & ---%$\times$1.0
    & 40.04	
    & 88.68
    & .0157  
    & .340 
    & ---
    & ---
    & ---
    & ---\\
MT EfficientDeP
    % & Eff. 
    & 4.78
    & 20.82
    & $\times$1.2
    & 38.64	 
    & 88.49	
    & .0171	
    & .354 
    & -1.9	
    & -6.3	
    & -4.1	
    & 3.1\\
EdgeDeP 
    % & Eff. 
    & 16.50
    & 20.29
    & $\times$1.3
    & 46.52	
    & 90.61	
    & .0143	
    & .316
    & +9.2	
    & +7.9	
    & +8.5	
    & 0.9\\ 
% EdgeDeP+MRE
%     % & Eff. 
%     & 16.50
%     & 20.29
%     & $\times$1.3
%     & 42.36	
%     & 89.91	
%     & .0145	
%     & .232
%     & +3.6	
%     & +19.7		
%     & +11.7		
%     & 11.4\\ 
EdgeDeP+MRE
    & 16.50
    & 20.29
    & $\times$1.3
    & 46.83	
    & 90.56	
    & .0144
    & .304
    & +9.5		
    & +9.5		
    & +9.5		
    & 0.0\\
EdgeDeP+MRE (rw)
    & 16.50
    & 20.29
    & $\times$1.3
    & 46.11	
    & 90.47		
    & .0143	
    & .281
    & +8.6			
    & +13.3		
    & +10.9		
    & 3.3\\
% EdgeDeP+MRE+$P_{seg}$
%     % & Eff. 
%     & 16.50
%     & 20.29
%     & $\times$1.3
%     & 
%     & 	
%     & 
%     & 
%     & 
%     & 
%     & 	
%     &\\ 
% EdgeDeP+MRE+$P_{depth}$
%     % & Eff. 
%     & 16.50
%     & 20.29
%     & $\times$1.3
%     & 45.33	
%     & 90.41	
%     & .0141	
%     & .282
%     & +7.6
%     & +13.8	
%     & +10.7		
%     & 4.4\\ 

%%%%%%%%%%%%%%%
% EfficientDeP+MRE
%     % & Eff. 
%     & 4.78
%     & 20.82
%     & $\times$1.2
%     & 37.71	
%     & 88.49
%     & .0161
%     & .324
%     & -3.0	
%     & +1.3	
%     & -0.9	
%     & 3.0\\

% EfficientDeP+MRE+BAM
%     % & Eff. 
%     & 4.78
%     & 20.82
%     & $\times$1.2
%     & 38.89
%     & 88.63
%     & .0168	
%     & .324
%     & -1.5	
%     & -0.9	
%     & -1.2	
%     & 0.4\\

% EdgeDeP+MRE+BAM
%     % & Eff. 
%     & 16.50
%     & 20.29
%     & $\times$1.3
%     & 46.82		
%     & 90.58		
%     & .0141	
%     & .312
%     & +9.5		
%     & +9.4		
%     & +9.5		
%     & 0.1\\ 
    
% \midrule
% \midrule
% ST EfficientDeP
%     % & Eff. 
%     & 9.37$^\dag$ 
%     & 25.67
%     & ---%$\times$1.0
%     & 55.02	
%     & 92.29	
%     & .0116	 
%     & .168
%     & ---
%     & ---
%     & ---
%     & ---\\
% MT EfficientDeP
%     % & Eff. 
%     & 4.78
%     & 20.82
%     & $\times$1.2
%     & 53.80	
%     & 91.94	
%     & .0124	
%     & .159
%     & -1.3	
%     & -0.9	
%     & -1.1	
%     & 0.3\\
% NAS+MRE+BAM
%     % & Eff. 
%     & 9.37$^\dag$ 
%     & 25.67
%     & $\times$1.3
%     & 58.54	
%     & 92.78	
%     & .0117	
%     & .156
%     & +3.5	
%     & +3.1	
%     & +3.3	
%     & 0.3\\

\bottomrule
\end{tabular}
} % \resizebox
\end{table*}

==> tab/sota_cityscapes1.tex <==
\begin{table*}[!t]
\centering

\caption{
\textbf{CityScapes results for 19-class semantic segmentation and depth estimation} -- Best numbers are in \textbf{bold}, second best are \underline{underlined}. Measurements of prior works are from Table 8 and Table 11 in \cite{adashare}. The parameter count for our single-task EfficientDeP is 3.42M. \textit{ST} stands for single-tasks. \textit{MT} stands for multi-task. We multiply the FLOPs by the number of tasks for methods that need multiple runs to get different per-task predictions. FLOPs are giga(G) and numbers of parameters are in millions(M). Both are measured for 256x256 resolution.
% $^\dag$ means the measurement were summed over all tasks because the network performs one task at a time.
} % \caption
\label{tab:main_table}

\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}l|cc||cc|cc||cc|cc@{}}
\begin{tabular}{@{}lccc|cccc|ccc@{}}

\toprule

\multicolumn{1}{c}{}  
    & \multicolumn{3}{c}{Model} 
    & \multicolumn{2}{c}{Seg} 
    & \multicolumn{2}{c}{Depth} 
    & \multicolumn{3}{c}{Avg} \\

Method 
    % & Arch 
    & \#P
    & GFLOP
    % & Lat %this justifies the increase in flop of NAS models
    & Speed%$\uparrow$ 
    & mIoU 
    & PAcc 
    & AbsE 
    & RelE 
    % & $\Delta$Seg
    % & $\Delta$Depth
    & $\Delta T_{S}$
    & $\Delta T_{D}$
    % & Mean$\Delta$ 
    % & STD$\Delta$ \\
    & $\mu\Delta$
    % & $\sigma\Delta$ 
    \\

\midrule

ST R-A baseline \cite{adashare}  
    % & Res. 
    & 42.6
    & 87.1 %87.12 %66.70$^\dag$ 
    & ---
    % & ---
    & 40.20  
    & 74.70  
    & .0170 
    & .330 
    & ---
    & ---
    & ---
    % & ---
    \\
MT R-A baseline \cite{adashare} 
    % & Res. 
    & 21.3
    & 43.6
    & ---
    % & ---
    & 37.70 
    & 73.80 
    & .0180 
    & .340 
    & -3.7 
    & -4.5 
    & -4.1 
    % & \underline{0.5} 
    \\

Cross-Stitch \cite{cross_stitch} 
    % & Res. 
    & 42.6
    & 48.4%48.40 %37.06   
    & ---
    % & ---
    & 40.30 
    & 74.30 
    & .0150 
    & .300 
    & -0.1 
    & \textbf{+10.4} 
    & \textbf{+5.1} 
    % & 7.5 
    \\

Sluice \cite{sluice} 
    % & Res. 
    & 42.6
    & 48.4%48.40%37.06  
    & ---
    % & ---
    & 39.80 
    & 74.20 
    & .0160 
    & .310 
    & -0.8 
    & +6.0 
    & +2.6 
    % & 4.8 
    \\

NDDR-CNN \cite{nddr} 
    % & Res. 
    & 44.1
    & 50.1 %50.05%38.32  
    & ---
    % & ---
    & 41.50 
    & 74.20 
    & .0170 
    & .310 
    & +1.3 
    & +3.0 
    & +2.2 
    % & 1.2 
    \\

MTAN \cite{mtan} 
    % & Res. 
    & 51.3
    & 57.9 %57.87 %44.31  
    & ---
    % & ---
    & 40.80 
    & 74.30 
    & .0150 
    & .320 
    & +0.5 
    & \underline{+7.4} 
    & \underline{+3.9} 
    % & 4.9 
    \\
    
DEN \cite{nas_mt_cls_elastic} 
    % & Res. 
    & 23.9
    & 51.2 %51.17 %78.36$^\dag$  
    & ---
    % & ---
    & 38.00 
    & 74.20 
    & .0170 
    & .370 
    & -3.1 
    & -6.1 
    & -4.6 
    % & 2.1 
    \\

AdaShare \cite{adashare} 
    % & Res.  
    & 21.3
    & 87.1 %87.12 %66.70$^\dag$  
    & ---
    % & ---
    & 41.50 
    & 74.90 
    & .0160 
    & .330 
    & \underline{+1.8} 
    & +2.9 
    & +2.3 
    % & 0.8 
    \\

\midrule

ST R-B baseline 
    % & Res. 
    & 43.7
    & 19.7 %78.85$^\dag$ 
    % & 86.57
    & $\times$1.0
    & 41.04 
    & 89.05 
    & .0168    
    & .359
    & ---   
    & ---
    & ---
    % & --- 
    \\
    
MT R-B baseline 
    % & Res. 
    & 21.9
    & 9.9
    & $\times$1.7
    & {37.66}
    & {88.66}
    & {.0175}
    & {.371}
    & -4.3	 
    & -3.9	
    & -4.1	
    % & 0.3 
    \\

MT E-B baseline %EfficientDeP
    % & Eff. 
    & 3.4 %3.43
    & 1.2 %1.20
    % & 20.82
    & $\times$4.2
    & 38.64	 
    & 88.49	
    & .0171	
    & .354 
    & -3.2	
    & -0.2	
    & -1.7	
    % & 2.1
    \\

EDNAS %EdgeDeP
    % & Eff. 
    & 4.3 %4.32M
    & 4.1 %4.12M
    % & 20.29
    & $\times$4.3
    & 46.52	
    & 90.61	
    & .0143	
    & .316
    & +7.5		
    & +13.1
    & +10.3	
    % & 3.9
    \\ 

EDNAS+MRE (best $\sigma\Delta$)
    & 4.3 %4.32M
    & 4.1 %4.12M
    % & 20.29
    & $\times$4.3
    & 47.32	
    & 90.66	
    & .0160	
    & .316
    & +8.6	
    & +8.3	
    & +8.4	
    % & 0.2
    \\

EDNAS+MRE
    & 4.3 %4.32M
    & 4.1 %4.12M
    % & 20.29
    & $\times$4.3
    & 47.28	
    & 90.52	
    & .0161	
    & .298
    & +8.4	
    & +10.4	
    & +9.4	
    % & 1.4
    \\

% EDNAS+MRE
%     & 4.1 %4.12M
%     & 4.3 %4.32M
%     & 20.29
%     & $\times$4.3
%     & 47.54	
%     & 90.74	
%     & 0.0153	
%     & 0.308
%     & +8.9	
%     & +11.6	
%     & +10.2	
%     & 1.9\\

EDNAS+MRE (best $\mu\Delta$)
    & 4.3 %4.32M
    & 4.1 %4.12M
    % & 20.29
    & $\times$4.3
    & 46.11	
    & 90.47	
    & .0143	
    & .281
    & +7.0		
    & +18.2		
    & +12.6	
    % & 7.9
    \\

\midrule

ST E-B baseline %EfficientDeP
    % & Eff. 
    & 3.4 %3.42
    & 2.3 %2.34 %9.37$^\dag$ 
    % & 25.67
    & $\times$1.0
    & 40.04	
    & 88.68
    & .0157  
    & .340 
    & ---
    & ---
    & ---
    % & ---
    \\
MT E-B baseline %EfficientDeP
    % & Eff. 
    & 3.4 %3.43
    & 1.2 %1.20
    % & 20.82
    & $\times$1.2
    & 38.64	 
    & 88.49	
    & .0171	
    & .354 
    & -1.9	
    & -6.3	
    & -4.1	
    % & 3.1
    \\
EDNAS 
    % & Eff. 
    & 4.3 %4.32M
    & 4.1 %4.12M
    % & 20.29
    & $\times$1.3
    & 46.52	
    & 90.61	
    & .0143	
    & .316
    & +9.2	
    & +7.9	
    & +8.5	
    % & 0.9
    \\ 
EDNAS+MRE
    & 4.3 %4.32M
    & 4.1 %4.12M
    % & 20.29
    & $\times$\textbf{1.3}
    & \textbf{46.83}	
    & \underline{90.56}	
    & \underline{.0144}
    & \textbf{.304}
    & +\textbf{9.5}	
    & +\textbf{9.5}		
    & +\textbf{9.5}		
    % & \textbf{0.0}
    \\
EDNAS+MRE (rw)
    & 4.3 %4.32M
    & 4.1 %4.12M
    % & 20.29
    & $\times$1.3
    & 46.11	
    & 90.47		
    & \textbf{.0143}
    & \textbf{.281}
    & +8.6			
    & \textbf{+13.3}	
    & \textbf{+10.9}		
    % & 3.3
    \\

\bottomrule
\end{tabular}
} % \resizebox
\end{table*}

==> tab/sota_nyuv2.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccccc@{}}
\toprule
%
% Method & seg & depth & norm & keypoint & edge & mean $\delta$ \\
% \midrule
% Single task & 0 & 0 & 0 & 0 & 0\\
% Prior Single-task Baseline & \\
% Prior Multi-task Baseline & \\
% MTAN & \\
% AdaShare & \\
% Our Single-task Baseline & \\
% Our Multi-task Baseline & \\
% Our NAS+MT& \\
%
Method & seg & depth & norm  & $\Delta$ Mean & $\Delta$ STD\\
\midrule
Single task & 0 & 0 & 0 & 0 & 0\\
Multi-task  & \\
EMNAS       & \\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
\textbf{NYUv2 dataset for Seg+Depth+Norm+KeyP+Edge} -- Text description here
} % \caption
\label{tab:sota_nyuv2}
\end{table}

==> tab/stronger_baseline.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lcccccc@{}}
    \toprule
    Method & GFLOPs & miou (seg) & abs error (depth) & $\delta$ seg & $\delta$ depth & $\delta$ avg \\
    \midrule
    % MTAN Single-task &  & 51.09 &  0.0158 &  \\
    % MTAN Multi-task &  & 51.21 & 0.0158 &  \\
    Deeplab-ResNet Single-task \cite{adashare} & 33.35 & 40.20 & 0.01700 &  \\
    Deeplab-ResNet Multi-task \cite{adashare} & 33.35 & 37.70 & 0.01800 & -6.22\% & -5.88\% & -6.05\%\\
    AdaShare \cite{adashare} & 33.35 & 41.50 & 0.01600\\
    Our Single-task & 2.35 & 57.20 & 0.01198 &  \\
    Our Single-task & 2.35 & 55.78 & 0.01187 & -2.48\% & +0.92\% & -0.78\% \\
    \bottomrule
\end{tabular}
} % \resizebox
\caption{
\textbf{Stronger baseline on CityScapes} -- Text description here
} % \caption
\label{tab:stronger_baseline}
\end{table}

==> tab/transfer_cityscapes.tex <==
\begin{table*}
\centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
% \toprule
% Method & \delta miou (seg) & \delta abs error (depth) & \delta avg all tasks \\
% \midrule
% Single task & 0 & 0 & 0 \\
% NAS+Seg \xrightarrow{} MT & ~ & ~ & ~ \\
% NAS+Depth \xrightarrow{} MT & +0.5 & +0.9 & +0.7 \\
% NAS+MT(ours) & +2.3 & +2.1 & +2.2 \\
% \bottomrule
% \end{tabular}
% } % \resizebox
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}l||cc|cc||cc|cc@{}}
\toprule
        \multicolumn{1}{c}{} & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} & \multicolumn{4}{c}{Overall} \\
Method & mIoU & PixAcc & AbsErr & RelErr & $\Delta$Seg & $\Delta$Depth  & Mean$\Delta$ & STD$\Delta$ \\
\midrule %========================================================
% ST EfficientDeP &
%     55.02 & 92.29 & 0.01198   & 0.2716 & --    & -- & --   & --\\
% MT EfficientDeP &
%     53.53	& 91.94	& 0.01187 & 0.2808 & -1.5  & -1.2 & -1.4 & 0.2\\
% NAS-D $\xrightarrow{}$ MT &
%     56.16	& 92.40	& 0.01148	& 0.2746 & +1.1	& +1.5 & +1.3	& 0.3 \\
% NAS-S $\xrightarrow{}$ MT & 
%     56.65	& 92.54 & 0.01133	& 0.2721 & +1.6	& +2.6 & +2.1	& 0.7 \\
% EMNAS &
%     56.94 & 92.47 & 0.01137   & 0.2727 & +1.8 & +2.3 & +2.1 & 0.4\\
%
ST EfficientDeP & 
    {55.02} & {92.29} & \textbf{0.01155}   & 0.1681 & 0.0    & 0.0 & 0.0  & 0.0 \\
MT EfficientDeP & 
    53.80	& 91.94	& {0.01241} & {0.1586} & -1.3   & -0.9  & -1.1 & \underline{0.3}\\
NAS-Seg $\xrightarrow{}$ MT & 
    \underline{58.17}&	\textbf{92.78}&	0.01176&	\underline{0.1557} & \underline{+3.1} &	\underline{+2.8} &	\underline{+3.0} &	\textbf{0.2}\\
NAS-Depth $\xrightarrow{}$ MT & 
    57.97&	\underline{92.73}&	0.01189&	0.1577 & +2.9&	+1.6 	&+2.3	&0.9 \\
EMNAS & 
    \textbf{58.54} & \textbf{92.78} & \underline{0.01170}   & \textbf{0.1556} & \textbf{+3.5} & \textbf{+3.1} & \textbf{+3.3} & \underline{0.3}\\ 
\bottomrule
\end{tabular}
% } % \resizebox
\caption{
\textbf{EMNAS vs. Transferring single-task NAS} -- We compare EMNAS with the transferring of single-task NAS' models to multi-task settings on CityScapes
} % \caption
\label{tab:transfer_cityscapes}
% \vspace{-1em}
\end{table*}

==> tab/transfer_nyuv2.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & seg & depth & norm & keypoint & edge & \delta avg all tasks \\
\midrule
Single task & 0 & 0 & 0 & 0 & 0\\
NAS+Seg \xrightarrow{} MT &\\
NAS+Depth \xrightarrow{} MT & \\
NAS+MT(ours) & \\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
\textbf{NYUv2 dataset for Seg+Depth+Norm+KeyP+Edge} -- Text description here
} % \caption
\label{tab:transfer_nyuv2}
\end{table}

==> tab/x_arch_found.tex <==
\begin{table}
\centering

\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\subfloat[Depth-only Arch. found by Single-Task NAS]{
    \begin{tabular}{@{}cccccc@{}}
        \toprule
        No. & Layer & Stride & Kernel & Filters & Expansion \\
        \midrule
        0 & Conv2D & 2 & 3 & 32  & -- \\
        1 & FusedIBN & 1 & 3 & 24  & 1 \\
        2 & IBN & 2 & 3 & 36  & 6 \\
        3 & IBN & 1 & 3 & 36  & 6 \\
        4 & FusedIBN & 2 & 5 & 40  & 6 \\
        5 & FusedIBN & 1 & 5 & 40  & 3 \\
        6 & IBN & 2 & 3 & 80  & 6 \\
        7 & FusedIBN & 1 & 3 & 120 & 3 \\
        8 & FusedIBN & 1 & 3 & 80  & 6 \\
        9 & FusedIBN & 1 & 3 & 168 & 3 \\
        10 & FusedIBN & 1 & 3 & 56  & 6 \\
        11 & FusedIBN & 1 & 3 & 112 & 3 \\
        12 & FusedIBN & 2 & 5 & 192 & 6 \\
        13 & FusedIBN & 1 & 3 & 192 & 6 \\
        14 & IBN & 1 & 5 & 192 & 3 \\
        15 & IBN & 1 & 5 & 192 & 3 \\
        16 & FusedIBN & 1 & 5 & 240 & 3 \\
        \bottomrule
    \end{tabular}
}
\quad
\subfloat[Seg+Depth Arch. found by EDNAS]{
    \begin{tabular}{@{}cccccc@{}}
        \toprule
        No. & Layer & Stride & Kernel & Filters & Expansion \\
        \midrule
        0 & Conv2D & 2 & 3 & 32  & -- \\
        1 & FusedIBN & 1 & 3 & 16  & 1 \\
        2 & IBN & 2 & 5 & 36  & 6 \\
        3 & FusedIBN & 1 & 5 & 24  & 6 \\
        4 & FusedIBN & 2 & 3 & 60  & 6 \\
        5 & FusedIBN & 1 & 3 & 40  & 3 \\
        6 & FusedIBN & 2 & 5 & 120 & 3 \\
        7 & IBN & 1 & 3 & 120 & 3 \\
        8 & FusedIBN & 1 & 5 & 80  & 6 \\
        9 & FusedIBN & 1 & 5 & 168 & 6 \\
        10 & FusedIBN & 1 & 5 & 84  & 3 \\
        11 & FusedIBN & 1 & 5 & 84  & 6 \\
        12 & FusedIBN & 2 & 5 & 288 & 3 \\
        13 & FusedIBN & 1 & 3 & 96  & 3 \\
        14 & FusedIBN & 1 & 3 & 96  & 6 \\
        15 & FusedIBN & 1 & 3 & 96  & 3 \\
        16 & FusedIBN & 1 & 5 & 160 & 6 \\
        \bottomrule
    \end{tabular}
}
} % \resizebox

\caption{
\textbf{Backbone Architecture found by EDNAS.} 
This table summarized the backbone architecture found EDNAS for multi-task segmentation and depth estimation on CityScapes
% , same model as presented in Table \ref{tab:main_table}.
The first Conv2D layer is a fixed stem following by 16 tunable layers.
% Figure \ref{fig:ibn_v_fused} visualized the difference between IBN and FusedIBN blocks
} % \caption
\label{tab:arch_found}

% \vspace{-2em}
\end{table}

==> tab/x_nyu_sdn_baselines.tex <==
\begin{table*}[t]
\centering

\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}l|c||cc|cc|cccc||ccc|cc@{}}
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\multicolumn{1}{c}{}  
    % &\multicolumn{1}{c}{} 
    & \multicolumn{2}{c}{Seg} 
    & \multicolumn{2}{c}{Depth} 
    & \multicolumn{4}{c}{Surface Normal} 
    & \multicolumn{4}{c}{Avg} 
    \\
Method 
    % & FLOPs 
    & mIoU 
    & PAcc 
    & AbsE 
    & RelE 
    & MeanE 
    & $\theta$11 
    & $\theta$22 
    & $\theta$30  
    & $\Delta T_{S}$
    & $\Delta T_{D}$
    & $\Delta T_{SN}$
    & $\Delta T$
    % & STD$\Delta$ 
    \\

\midrule

ST baseline \cite{adashare}
	& 27.5
	& 58.9
	& 0.62
	& 0.25
	& 17.5
	& 34.9
	& 73.3
	& 85.7
	& ---
	& ---
	& ---
	& ---
	\\
MT baseline \cite{adashare}
	& 24.1
	& 57.2
	& 0.58
	& 0.23
	& 16.6
	& 42.5
	& 73.2
	& 84.6
	& -7.6
	& +7.2
	& +6.4
	& {+2.0}
	\\

Cross-Stitch \cite{cross_stitch}
    % &55.59G 
    & 25.4 & 57.6 & 0.58 & 0.23 & 17.2 & 41.4 & 70.5 & 82.9 & -4.9 & +7.2 & +3.3 & +1.9 
    % & 6.2 
    \\
Sluice \cite{sluice} 
    % &55.59G 
    & 23.8 & 56.9 & 0.58 & 0.24 & 17.2 & 38.9 & 71.8 & 83.9 
    & -8.4 & +5.2 & +2.3 & -0.3 
    % & 7.2 
    \\
NDDR-CNN \cite{nddr} 
    % &57.21G 
    & 21.6 & 53.9 & 0.66 & 0.26 & 17.1 & 37.4 & 73.7 & 85.6 & -15.0 & -5.2 & +2.5 & -5.9 
    % & 8.7 
    \\
MTAN \cite{mtan}
    % &58.43G 
    & 26.0 & 57.2 & 0.57 & 0.25 & 16.6 & 43.7 & 73.3 & 84.4 & -4.2 & +4.0 
    & \textbf{+7.2} & +2.4 \
    % & 5.9 
    \\
DEN \cite{nas_mt_cls_elastic} 
    % &173.1G$^\dag$ 
    & 23.9 & 54.9 & 0.97 & 0.31 & 17.1 & 36.0 & 73.4 & 85.9 & -9.9 & -40.2 & +1.5 & -16.2 
    % & 21.5 
    \\

AdaShare \cite{adashare}
	& 30.2
	& 62.4
	& 0.55
	& 0.20
	& 16.6
	& 45.0
	& 71.7
	& 83.0
	& \textbf{+7.9}
	& \textbf{+15.6}
	& \textbf{+7.2}
	& \textbf{+10.2}
	\\

\midrule

ST edge baseline
	& 23.1
	& 58.3
	& 0.50
	& 0.20
	& 13.8
	& 50.8
	& 81.2
	& 90.8
	& ---
	& ---
	& ---
	& ---
	\\
MT edge baseline
	& 19.5
	& 54.8
	& 0.55
	& 0.22
	& 16.5
	& 41.9
	& 73.0
	& 85.1
	& -10.7
	& -10.0
	& -13.3
	& {-11.3}
	\\
EDNAS 
	& 22.1
	& 57.7
	& 0.51
	& 0.20
	& 14.3
	& 49.5
	& 79.2
	& 89.4
	& -2.5	
	& -1.3	
	& -2.6	
	& {-2.1}
	\\
EDNAS+MRE 
	& 22.1
	& 58.1
	& 0.51
	& 0.20
	& 12.6
	& 56.1
	& 83.9
	& 92.4
	& -2.3
	& -0.9
	& +6.0
	& {+0.9}
	\\
\bottomrule
\end{tabular}
} % \resizebox

\caption{
\textbf{Three-task NYU-v2 results compared to ST baseline.}
Our tasks of interest include 40-class semantic segmentation, depth estimation, and surface normal estimation. Best numbers are in \textbf{bold}.
% , second best are underlined.
\textit{ST} stands for single-task and \textit{MT} stands for multi-task.
% while the edge latencies are measured with 256$\times$256 resolution due to device limitations.
We multiply the FLOPs by the number of tasks for methods that need multiple runs to get different per-task predictions.
The measurements of prior works are from Table 9 and Table 11 in \cite{adashare}
% These methods uses ResNet-Deeplab/ASPP backbone, as opposed to EfficientNet-BiFPN base used by our EfficientDeP and EMNAS-found models
} % \caption
\label{tab:nyu_sdn_baselines}

% \vspace{-0.5em}
\end{table*}


==> tab/x_nyu_segdepth.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}l|cccc||cc|cc||cc|cc@{}}
% \toprule
%         \multicolumn{1}{c}{}  &\multicolumn{4}{c}{Architecture} & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} & \multicolumn{4}{c}{Overall} \\
% Method & Base & \#Param & \#FLOPs & Edge Lat & mIoU & PixAcc & AbsErr & RelErr & $\Delta$Seg(v.*) & $\Delta$Depth(v.*) & Mean$\Delta$(v.*) & STD$\Delta$ \\

% \midrule
% ST baseline* \cite{adashare}  & R-A & -- & 36.96G$^\dag$  
%     & -- & 27.5 & 58.9 & 0.62 & 0.25 & 0.0    & 0.0    & 0.0   & 0.0\\

% AdaShare \cite{adashare} & R-A & -- & 36.96G$^\dag$  
%     & -- & 30.2 & 62.4 & 0.55 &  0.20 & +7.9 & +15.6 & +11.8	 & 5.5 \\

% \midrule
% ST EfficientDeP & E-B & 3.42M & 9.40G$^\dag$ & 38.69ms$^\dag$
%      & 30.55 & 62.12 & 0.4796 & 0.1883 & 0.0 (+8)    & 0.0 (+24) & 0.0 (+16)   & 0.0 \\
% MT EfficientDeP & E-B & 3.43M & 4.81G & 34.00ms
%     & 30.48	& 62.45	& 0.4712 & 0.1829
%     & +0.1 (+8)  & +2.3 (+25) & +1.2 (+17) & 1.5\\
% EMNAS & E-B & 3.26M &	7.85G &	33.49ms	
%     &31.69	&63.21	&0.4661	&0.1806
%     &+2.7(+11)	&+3.4(+26)	&+3.1(+19)	&0.5 \\ 
% \bottomrule
% \end{tabular}
%
%%%% Without #Param column
\begin{tabular}{@{}l|ccc||cc|cc||cc|cc@{}}
\toprule
        \multicolumn{1}{c}{}  &\multicolumn{3}{c}{Architecture} & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} & \multicolumn{4}{c}{Overall} \\
Method & Base & \#FLOPs & Edge Lat & mIoU & PixAcc & AbsErr & RelErr & $\Delta$Seg(v.*) & $\Delta$Depth(v.*) & Mean$\Delta$(v.*) & STD$\Delta$ \\

\midrule
ST baseline* \cite{adashare}  & R-A & 36.96G$^\dag$  
    & -- & 27.5 & 58.9 & 0.62 & 0.25 & 0.0    & 0.0    & 0.0   & 0.0\\

AdaShare \cite{adashare} & R-A & 36.96G$^\dag$  
    & -- & 30.2 & 62.4 & 0.55 &  0.20 & +7.9 & +15.6 & +11.8	 & 5.5 \\

\midrule
ST EfficientDeP & E-B & 9.40G$^\dag$ & 38.69ms$^\dag$
     & 30.55 & 62.12 & 0.4796 & 0.1883 & 0.0 (+8)    & 0.0 (+24) & 0.0 (+16)   & 0.0 \\
MT EfficientDeP & E-B & \textbf{4.81}G & 34.00ms
    & 30.48	& 62.45	& 0.4712 & 0.1829
    & +0.1 (+8)  & +2.3 (+25) & +1.2 (+17) & 1.5\\
EMNAS & E-B &	7.85G &	\textbf{33.49ms}	
    &\textbf{31.69}	&\textbf{63.21}	&\textbf{0.4661}	&\textbf{0.1806}
    &\textbf{+2.7}(\textbf{+11})
    &\textbf{+3.4}(\textbf{+26})
    &\textbf{+3.1}(\textbf{+19})	
    &\textbf{0.5} \\ 
\bottomrule
\end{tabular}
} % \resizebox
\caption{
\textbf{2-task NYU-v2 results for 40-class semantic segmentation and depth estimation} -- Best numbers are in bold. 
% second best are \underline{underlined}. 
\textit{ST} stands for single-task, \textit{MT} stands for multi-task, \textit{R-A} stands for ResNet-ASPP, and \textit{E-B} stands for EfficientNet-BiFPN.
We calculate our models' FLOPs using the training resolution of 512$\times$512, while the edge latencies are measured with 256$\times$256 resolution due to device limitations.
We multiply the FLOPs by the number of tasks for methods that need multiple runs to get different per-task predictions, denoted by$^\dag$. 
The parameter count for our single-task EfficientDeP is 3.42M.
The measurements of \textit{ST Baseline} and \textit{AdaShare} are from Table 9 and Table 11 in \cite{adashare}. 
Particularly, AdaShare's numbers are lower bound approximations adopted from their 3-task experiment, included for reference.
} % \caption
\label{tab:nyu_segdepth}
% \vspace{-0.5em}
\end{table*}


==> tab/x_nyu_segdepthnorm0.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line

% \begin{tabular}{@{}l|c||cc|cc|cccc||ccc|cc@{}}
\begin{tabular}{@{}lcccccccccccccc@{}}
\toprule
        \multicolumn{1}{c}{}  &\multicolumn{1}{c}{} & \multicolumn{2}{c}{Seg} & \multicolumn{2}{c}{Depth} & \multicolumn{4}{c}{Surface Normal} & \multicolumn{5}{c}{Overall} \\
Method 
    & FLOPs 
    & mIoU 
    & PAcc 
    & AbsE 
    & RelE 
    & MeanE 
    & $\theta$11 
    & $\theta$22 
    & $\theta$30  
    & $\Delta$S
    & $\Delta$D
    & $\Delta$SN
    & Mean$\Delta$
    & STD$\Delta$ \\

\midrule
ST Baseline* \cite{adashare}  
    % & R-A 
    & 150.4G$^\dag$ 
    & 27.5 & 58.9 
    & 0.62 & 0.25 
    &17.5	&34.9	&73.3	&85.7
    & ---    & --- & --- 
    & ---   & ---\\

% MT baseline \cite{adashare}
%     & 50.13G 
%     & 24.1	&57.2	
%     &0.58	&0.23	
%     &16.6	&42.5	&73.2	&84.6
%     & --    & -- & -- 
%     & --   & --\\

MT Baseline \cite{adashare}
    & 50.13G & 24.1 & 57.2 & 0.58 & 0.23 & 16.6 & 42.5 & 73.2 & 84.6 & -7.6 & 7.2 & 6.4 & 2.0 & 8.3 \\

Cross-Stitch \cite{cross_stitch}
    &55.59G & 25.4 & 57.6 & 0.58 & 0.23 & 17.2 & 41.4 & 70.5 & 82.9 & -4.9 & 7.2 & 3.3 & 1.9 & 6.2 \\
Sluice \cite{sluice} 
    &55.59G & 23.8 & 56.9 & 0.58 & 0.24 & 17.2 & 38.9 & 71.8 & 83.9 & -8.4 & 5.2 & 2.3 & -0.3 & 7.2 \\
NDDR-CNN \cite{nddr} 
    &57.21G & 21.6 & 53.9 & 0.66 & 0.26 & 17.1 & 37.4 & 73.7 & 85.6 & -15.0 & -5.2 & 2.5 & -5.9 & 8.7 \\
MTAN \cite{mtan}
    &58.43G & 26.0 & 57.2 & 0.57 & 0.25 & 16.6 & 43.7 & 73.3 & 84.4 & -4.2 & 4.0 & 7.2 & 2.4 & 5.9 \\
DEN \cite{nas_mt_cls_elastic} 
    &173.1G$^\dag$ 
    & 23.9 & 54.9 & 0.97 & 0.31 & 17.1 & 36.0 & 73.4 & 85.9 & -9.9 & -40.2 & 1.5 & -16.2 & 21.5 \\
AdaShare \cite{adashare} 
    &150.4G$^\dag$ 
    & {30.2} & \underline{62.4} & 0.55 
    &\underline{0.20} & 16.6 & 45.0 & 71.7 & 83.0 & 7.9 & 15.6 & 7.2 & 10.2 & 4.7 \\

\midrule
    
ST Edge Baseline
    & \todo{14.08G$^\dag$}
    & 23.08	
    & 58.27	
    & 0.50	
    & 0.20	
    & 13.79	
    & 50.79	
    & 81.20	
    & 90.78	
    & ---
    & ---
    & ---
    & ---
    & ---
    \\ 
MT Edge Baseline
    & \todo{4.89G}
    & 19.5	
    & 54.8	
    & 0.548	
    & 0.22	
    & 16.5	
    & 41.9	
    & 73.0	
    & 85.1
    & -10.7	
    & -10.0	
    & -13.3	
    & -11.3	
    & 1.8\\
EMNAS
    & \todo{9.52G}
    & 22.1	
    & 57.7	
    & 0.508	
    & 0.20	
    & 14.3	
    & 49.5	
    & 79.2	
    & 89.4
    & -2.5	
    & -1.3	
    & -2.6	
    & -2.1	
    & 0.7\\
EMNAS+MRE
    & \todo{9.52G}
    & 22.1	
    & 58.1	
    & 0.509	
    & 0.20	
    & 12.6	
    & 56.1	
    & 83.9	
    & 92.4
    & -2.3	
    & -0.9	
    & +6.0	
    & +0.9	
    & 4.4\\
        
\bottomrule
\end{tabular}
} % \resizebox
\caption{
\textbf{3-task NYU-v2 results for 40-class segmentation, depth estimation, and surface normal estimation} -- Best numbers are in bold, second best are underlined.
\textit{ST} stands for single-task and \textit{MT} stands for multi-task.
\textit{EfficientDeP-R} and \textit{EMNAS-R} denote models trained with reweighted loss terms to prioritize segmentation and depth estimation gains.
% The \textit{R-A} stands for ResNet-ASPP, and \textit{E-B} stands for EfficientNet-BiFPN.
We calculate our models' FLOPs using the training resolution of 512$\times$512. 
% while the edge latencies are measured with 256$\times$256 resolution due to device limitations.
We multiply the FLOPs by the number of tasks for methods that need multiple runs to get different per-task predictions, denoted by$^\dag$. 
The parameter count for our single-task EfficientDeP is 3.42M and the count for the reported EMNAS model is 3.79M.
The measurements of prior works are from Table 9 and Table 11 in \cite{adashare}. These methods uses ResNet-Deeplab/ASPP backbone, as opposed to EfficientNet-BiFPN base used by our EfficientDeP and EMNAS-found models.
} % \caption
\label{tab:nyu_segdepthnorm}
% \vspace{-0.5em}
\end{table*}


==> tab/x_nyu_segdepthnorm1.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line

% \begin{tabular}{@{}l|c||cc|cc|cccc||ccc|cc@{}}
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
\multicolumn{1}{c}{}  
    % &\multicolumn{1}{c}{} 
    & \multicolumn{2}{c}{Seg$\Delta$} 
    & \multicolumn{2}{c}{Depth$\Delta$} 
    & \multicolumn{4}{c}{Surface Normal$\Delta$} 
    & \multicolumn{5}{c}{Overall} 
    \\
Method 
    % & FLOPs 
    & mIoU 
    & PAcc 
    & AbsE 
    & RelE 
    & MeanE 
    & $\theta$11 
    & $\theta$22 
    & $\theta$30  
    & $\Delta$S
    & $\Delta$D
    & $\Delta$SN
    & Mean$\Delta$
    & STD$\Delta$ \\

\midrule

MT Baseline \cite{adashare}
    &-12.4
	&-2.9
	&+6.5
	&+8.0
	&+5.1
	&+21.8
	&-0.1
	&-1.3
	&-7.6
	&+7.2
	&+6.4
	&+2.0
	&+8.3
	\\
Cross-Stitch \cite{cross_stitch}
	&-7.6
	&-2.2
	&+6.5
	&+8.0
	&+1.7
	&+18.6
	&-3.8
	&-3.3
	&-4.9
	&+7.2
	&+3.3
	&+1.9
	&+6.2
    \\
Sluice \cite{sluice} 
	&-13.5
	&-3.4
	&+6.5
	&+4.0
	&+1.7
	&+11.5
	&-2.0
	&-2.1
	&-8.4
	&+5.2
	&+2.3
	&-0.3
	&+7.2
    \\
NDDR-CNN \cite{nddr} 
	&-21.5
	&-8.5
	&-6.5
	&-4.0
	&+2.3
	&+7.2
	&+0.5
	&-0.1
	&-15.0
	&-5.2
	&+2.5
	&-5.9
	&+8.7
    \\
MTAN \cite{mtan}
	&-5.5
	&-2.9
	&+8.1
	&+0.0
	&+5.1
	&+25.2
	&+0.0
	&-1.5
	&-4.2
	&+4.0
	&+7.2
	&+2.4
	&+5.9
    \\
DEN \cite{nas_mt_cls_elastic} 
	&-13.1
	&-6.8
	&-56.5
	&-24.0
	&+2.3
	&+3.2
	&+0.1
	&+0.2
	&-9.9
	&-40.2
	&+1.5
	&-16.2
	&+21.5
    \\
AdaShare \cite{adashare} 
	&+9.8
	&+5.9
	&+11.3
	&+20.0
	&+5.1
	&+28.9
	&-2.2
	&-3.2
	&+7.9
	&+15.6
	&+7.2
	&+10.2
	&+4.7
    \\

\midrule

MT Edge Baseline
	&-15.5
	&-5.9
	&-9.5
	&-10.4
	&-19.5
	&-17.6
	&-10.1
	&-6.2
	&-10.7
	&-10.0
	&-13.3
	&-11.3
	&+1.8
    \\
EMNAS
	&-4.1
	&-0.9
	&-1.4
	&-1.2
	&-3.7
	&-2.5
	&-2.5
	&-1.6
	&-2.5
	&-1.3
	&-2.6
	&-2.1
	&+0.7
    \\
EMNAS+MRE
	&-4.3
	&-0.2
	&-1.6
	&-0.2
	&+8.5
	&+10.4
	&+3.3
	&+1.8
	&-2.3
	&-0.9
	&+6.0
	&+0.9
	&+4.4
    \\
        
\bottomrule
\end{tabular}
} % \resizebox
\caption{
\textbf{3-task NYU-v2 results for 40-class segmentation, depth estimation, and surface normal estimation} -- Best numbers are in bold, second best are underlined.
\textit{ST} stands for single-task and \textit{MT} stands for multi-task.
\textit{EfficientDeP-R} and \textit{EMNAS-R} denote models trained with reweighted loss terms to prioritize segmentation and depth estimation gains.
% The \textit{R-A} stands for ResNet-ASPP, and \textit{E-B} stands for EfficientNet-BiFPN.
We calculate our models' FLOPs using the training resolution of 512$\times$512. 
% while the edge latencies are measured with 256$\times$256 resolution due to device limitations.
We multiply the FLOPs by the number of tasks for methods that need multiple runs to get different per-task predictions, denoted by$^\dag$. 
The parameter count for our single-task EfficientDeP is 3.42M and the count for the reported EMNAS model is 3.79M.
The measurements of prior works are from Table 9 and Table 11 in \cite{adashare}. These methods uses ResNet-Deeplab/ASPP backbone, as opposed to EfficientNet-BiFPN base used by our EfficientDeP and EMNAS-found models.
} % \caption
\label{tab:nyu_segdepthnorm}
% \vspace{-0.5em}
\end{table*}


==> tab/x_nyu_segdepthnorm_eccv.tex <==
\begin{table*}[t]
\centering

\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}l|c||cc|cc|cccc||ccc|cc@{}}
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\multicolumn{1}{c}{}  
    % &\multicolumn{1}{c}{} 
    & \multicolumn{2}{c}{Seg} 
    & \multicolumn{2}{c}{Depth} 
    & \multicolumn{4}{c}{Surface Normal} 
    & \multicolumn{4}{c}{Avg} 
    \\
Method 
    % & FLOPs 
    & $\Delta$mIoU 
    & $\Delta$PAcc 
    & $\Delta$AbsE 
    & $\Delta$RelE 
    & $\Delta$MeanE 
    & $\Delta \theta$11 
    & $\Delta \theta$22 
    & $\Delta \theta$30  
    & $\Delta T_{S}$
    & $\Delta T_{D}$
    & $\Delta T_{SN}$
    & $\Delta T$
    % & STD$\Delta$ 
    \\

\midrule

Cross-Stitch \cite{cross_stitch}
	&+5.4
	&+0.7
	&+0.0
	&+0.0
	&-3.6
	&-2.6
	&-3.7
	&-2.0
	&+3.0
	&+0.0
	&-3.0
	&+0.0
	\\
Sluice \cite{sluice} 	
	&-1.2
	&-0.5
	&+0.0
	&-4.3
	&-3.6
	&-8.5
	&-1.9
	&-0.8
	&-0.9
	&-2.2
	&-3.7
	&-2.3
	\\
NDDR-CNN \cite{nddr} 
	&-10.4
	&-5.8
	&-13.8
	&-13.0
	&-3.0
	&-12.0
	&+0.7
	&+1.2
	&-8.1
	&-13.4
	&-3.3
	&-8.3
	\\
MTAN \cite{mtan}
	&+7.9
	&+0.0
	&+1.7
	&-8.7
	&+0.0
	&+2.8
	&+0.1
	&-0.2
	&+3.9
	&-3.5
	&+0.7
	&+0.4
	\\
DEN \cite{nas_mt_cls_elastic} 
	&-0.8
	&-4.0
	&-67.2
	&-34.8
	&-3.0
	&-15.3
	&+0.3
	&+1.5
	&-2.4
	&-51.0
	&-4.1
	&-19.2
	\\
AdaShare \cite{adashare} 
	&\textbf{+25.3}
	&\textbf{+9.1}
	&+5.2
	&\textbf{+13.0}
	&+0.0
	&+5.9
	&-2.0
	&-1.9
	&\textbf{+17.2}
	&\textbf{+9.1}
	&+0.5
	&+8.9
	\\

\midrule

EDNAS
	&\underline{+13.4}
	&+5.3
	&\textbf{+7.5}
	&+8.4
	&\underline{+13.2}
	&\underline{+18.3}
	&\underline{+8.5}
	&\underline{+5.0}
	&+9.4
	&+7.9
	&\underline{+11.2}
	&\underline{+9.5}
	\\
EDNAS+MRE
	&+13.2
	&\underline{+6.0}
	&\underline{+7.2}
	&\underline{+9.2}
	&\textbf{+23.4}
	&\textbf{+34.0}
	&\textbf{+15.0}
	&\textbf{+8.5}
	&\underline{+9.6}
	&\underline{+8.2}
	&\textbf{+20.2}
	&\textbf{+12.7}
	\\

\bottomrule
\end{tabular}
} % \resizebox

\caption{
\textbf{Three-task NYU-v2 results compared to MT baseline.} 
% for 40-class segmentation, depth estimation, and surface normal estimation
Best numbers are in \textbf{bold}, second best are \textit{underlined}
% \textit{ST} stands for single-task and \textit{MT} stands for multi-task.
% \textit{EfficientDeP-R} and \textit{EMNAS-R} denote models trained with reweighted loss terms to prioritize segmentation and depth estimation gains.
% % The \textit{R-A} stands for ResNet-ASPP, and \textit{E-B} stands for EfficientNet-BiFPN.
% We calculate our models' FLOPs using the training resolution of 512$\times$512. 
% % while the edge latencies are measured with 256$\times$256 resolution due to device limitations.
% We multiply the FLOPs by the number of tasks for methods that need multiple runs to get different per-task predictions, denoted by$^\dag$. 
% The parameter count for our single-task EfficientDeP is 3.42M and the count for the reported EMNAS model is 3.79M.
% The measurements of prior works are from Table 9 and Table 11 in \cite{adashare}. These methods uses ResNet-Deeplab/ASPP backbone, as opposed to EfficientNet-BiFPN base used by our EfficientDeP and EMNAS-found models
} % \caption
\label{tab:nyu_segdepthnorm}

% \vspace{-0.5em}
\end{table*}

